Dark Kinetic Heating of Neutron Stars from Contact Interactions with Relativistic Targets

Dark matter can capture in neutron stars from scattering off ultra-relativistic electrons. We present a method to calculate the capture rate on degenerate targets with ultra-relativistic momenta in a compact astronomical object. Our treatment accounts for the target momentum and the Fermi degeneracy of the system. We derive scaling relations for scattering with relativistic targets and confirm consistency with the non-relativistic limit and Lorentz invariance. The potential observation of kinetic heating of neutron stars has a larger discovery reach for dark matter-lepton interactions than conventional terrestrial direct detection experiments. We map this reach onto a set of bosonic and fermionic effective contact interactions between dark matter and leptons as well as nucleons. We show the results for the contact operators up to dimension 6 for spin-0 and spin-1/2 dark matter interactions with relativistic as well as non-relativistic Standard Model fermions. Highlights of this program in the case of vector mediated interactions are presented in a companion letter [1]. Our method is generalizable to dark matter scattering in any degenerate medium where the Pauli exclusion principle leads to relativistic targets with a constrained phase space for scattering.

==> NeutronStarFermionBosonTable.tex <==
\begin{tabular}{lll}
\toprule
  Name 
  & Operator % $\times \Lambda^2$
  & $\Lambda^4|\mathcal{M}|^2$
  \; ($m_\chi^2 E_p^2$ term dominates when present)
  \\
\midrule
  $\mathcal{O}^\textnormal{F}_1$ 
  & $%y_\xi 
  \left(\bar{\chi}\chi\right) \left(\bar{\xi}\xi\right)$ 
  & $%y_\xi^2
  \left(4m_\chi^2-t\right)\left(4m_T^2-t\right)$
  \\
  $\mathcal{O}^\textnormal{F}_2$ 
  & $%y_\xi 
  \left(\bar{\chi} i\gamma^5\chi\right)\left(\bar{\xi}\xi\right)$ 
  & $%y_\xi^2 
  t\left(t-4m_T^2\right)$
  \\
  $\mathcal{O}^\textnormal{F}_3$ 
  & $%y_\xi 
  \left(\bar{\chi}\chi\right)\left(\bar{\xi} i\gamma^5\xi\right)$ 
  & $%y_\xi^2
  t\left(t-4m_\chi^2\right)$
  \\
  $\mathcal{O}^\textnormal{F}_4$ 
  & $%y_\xi 
  \left(\bar{\chi} i\gamma^5\chi\right)\left(\bar{\xi} i\gamma^5\xi\right)$ 
  & $%y_\xi^2 
  t^2$
  \\
  $\mathcal{O}^\textnormal{F}_5$ 
  & $\left(\bar{\chi}\gamma^\mu\chi\right)\left(\bar{\xi}\gamma_\mu\xi\right)$ 
  & 
  $4\left(m_T^2+m_\chi^2\right)^2
  -8s\left(m_T^2+m_\chi^2\right)
  +4s^2
  +4st
  +2t^2
  $
  \\
  $\mathcal{O}^\textnormal{F}_6$ 
  & $\left(\bar{\chi}\gamma^\mu\gamma^5\chi\right)\left(\bar{\xi}\gamma_\mu\xi\right)$ 
  & $
  4\left(m_T^2-m_\chi^2\right)^2
  -8s\left(m_T^2+m_\chi^2\right)
  -8\,t\,m_\chi^2
  +4s^2
  +4st
  +2t^2
  $
  \\
  $\mathcal{O}^\textnormal{F}_7$ 
  & $\left(\bar{\chi}\gamma^\mu\chi\right)\left(\bar{\xi}\gamma_\mu\gamma^5\xi\right)$ 
  & $
  4\left(m_T^2-m_\chi^2\right)^2
  -8s\left(m_T^2+m_\chi^2\right)
  -8\,t\,m_T^2
  +4s^2
  +4st
  +2t^2
  $
  \\
  $\mathcal{O}^\textnormal{F}_8$ 
  & $\left(\bar{\chi}\gamma^\mu\gamma^5\chi\right)\left(\bar{\xi}\gamma_\mu\gamma^5\xi\right)$ 
  & $
  4\left(m_T^4+10m_T^2m_\chi^2+m_\chi^4\right)
  -8(s+t)\left(m_T^2+m_\chi^2\right)
  +4s^2
  +4st
  +2t^2
  $
  \\
  $\mathcal{O}^\textnormal{F}_9$ 
  & $%y_\xi
  \left(\bar{\chi}\sigma^{\mu\nu}\chi\right)\left(\bar{\xi}\sigma_{\mu\nu}\xi\right)$ 
  & 
  $
  8%y_\xi^2
  \left[
    4\left(m_T^4+4m_T^2m_\chi^2+m_\chi^4\right)
    -2(4s+t)\left(m_T^2+m_\chi^2\right)
    +(2s+t)^2
    \right]
  $
  \\
  $\mathcal{O}^\textnormal{F}_{10}$ 
  & $%y_\xi 
  \left(\bar{\chi}\sigma^{\mu\nu}i\gamma^5\chi\right)\left(\bar{\xi}\sigma_{\mu\nu}\xi\right)$ 
  & 
  $
  8%y_\xi^2
  \left[
    4\left(m_T^2+m_\chi^2\right)^2
    -2(4s+t)\left(m_T^2+m_\chi^2\right)
    +(2s+t)^2
    \right]
  $
  \\
%
%% BOSONS
%
\midrule
    $\mathcal{O}^\textnormal{S}_1$ 
    & 
    $%y_\xi 
    \left(\chi^\dag\chi\right)
    \left(\bar\xi\xi\right)\Lambda$
    & 
    $
    %y_\xi^2
    \Lambda^2\left(4m_{\rm T}^2-t\right)
    $
    \\
    $\mathcal{O}^\textnormal{S}_2$ 
    & 
    $%y_\xi 
    \left(\chi^\dag\chi\right)
    \left( \bar\xi i\gamma^5 \xi \right) \Lambda$
    & $
    %y_\xi^2
    \Lambda^2\left(-t\right)
    $
    \\
    $\mathcal{O}^\textnormal{S}_3$ 
    & 
    % $\left(\chi^*_\nu\partial_\mu\chi^\nu\right)\left(\bar{\xi}\gamma^\mu\,\xi\right)$ 
    $
    \left( \chi^\dag i\partial_\mu \chi \right)
    \left( \bar\xi\gamma^\mu \xi \right)$
    & $
    4\left[\left(m_T^2+m_\chi^2\right)^2
    -2s\left(m_T^2+m_\chi^2\right)
    +s^2
    +st
    -m_{\rm T}^2t\right]
    $
    \\
    $\mathcal{O}^\textnormal{S}_4$ 
    & 
    % $\left(\chi^*_\mu\chi_\nu-\chi_\mu\chi^*_\nu\right)\left(\bar{\xi}\sigma^{\mu\nu}\,\xi\right)$ 
    $\left(\chi^\dag i \partial_\mu\chi\right)
    \left( \bar\xi\gamma^\mu\gamma^5 \xi \right)$
    & $
    4\left[\left(m_T^2-m_\chi^2\right)^2
    -2s\left(m_T^2+m_\chi^2\right)
    +s^2
    +st\right]
    $
    \\
\bottomrule
\bottomrule
\end{tabular}

==> NeutronStarPRDpreamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  COMMON PACKAGES  %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{graphicx}           % use \pdfoutput=1 after \documentclass
\usepackage[utf8]{inputenc}     % inspire bibs
\usepackage{aas_macros}				  % ads bibs
\usepackage{bm}                 % \boldsymbol
\usepackage{amsthm}
  \newtheoremstyle{mystyle}%    % Name
  {1em}%                           % Space above
  {1em}%                           % Space below
  {\itshape}%                   % Body font
  {}%                           % Indent amount
  {\bfseries}%                  % Theorem head font
  {.}%                          % Punctuation after theorem head
  { }%                          % Space after theorem head, ' ', or \newline
  {}%                           % Theorem head spec (can be left empty, meaning `normal')

\theoremstyle{mystyle}
  \newtheorem{thumb}{Rule of Thumb}
  \newtheorem{corollary}{Corollary of Thumb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  UNUSUAL PACKAGES        %%%%
%%%  Uncomment as necessary. %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% MATH AND PHYSICS SYMBOLS
%% ------------------------
\usepackage{slashed}				% \slashed{k}
\usepackage{mathrsfs}			 	% Weinberg-esque letters
\usepackage{bbm}					  % \mathbbm{1} conflict: XeLaTeX 
\usepackage{cancel}		
\usepackage[normalem]{ulem} 		% for \sout
%\usepackage{youngtab}	    		% Young Tableaux

%% FOR DRAFT EDITING AND DISCUSSION
\usepackage{lineno}
% \linenumbers          %% put this in main text

%% CONTENT FORMAT AND DESIGN
%% -------------------------
\usepackage[dvipsnames]{xcolor}
\usepackage[hang,flushmargin]{footmisc} % no footnote indent

\usepackage{fancyhdr}		% preprint number
\usepackage{lipsum}			% block of text 
\usepackage{framed}			% boxed remarks
\usepackage{subcaption}	% subfigures
\usepackage{cite}			  % group cites
\usepackage{xspace}			% macro spacing


%% TABLES IN LaTeX
%% ---------------
\usepackage{booktabs}		% professional tables
\usepackage{nicefrac}		% fractions in tables,
%\usepackage{multirow}		% multirow elements in a table
%\usepackage{arydshln}		% dashed lines in arrays

%% ARRAY STRETCH: vertical spacing between rows
% \renewcommand{\arraystretch}{1.5} %% put this in main text

%% Other Packages and Notes
%% ------------------------
\usepackage[font=small]{caption} % caption font is small
\usepackage{float}         % for strict placement e.g. [H]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  DOCUMENT PROPERTIES  %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[margin=2cm]{geometry}   % margins
\graphicspath{{figures/}}			% figure folder
\numberwithin{equation}{section}    % set equation numbering


%% References in two columns, small tex.stackexchange/20758/
\usepackage{multicol}
\usepackage{etoolbox}
\usepackage{relsize}
\patchcmd{\thebibliography}
  {\list}
  {\begin{multicols}{2}\smaller\list}
  {}
  {}
\appto{\endthebibliography}{\end{multicols}}


% Change list spacing (instead of package paralist)
% from: http://en.wikibooks.org/wiki/LaTeX/List_Structures#Line_spacing
\let\oldenumerate\enumerate
\renewcommand{\enumerate}{
  \oldenumerate
  \setlength{\itemsep}{2pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}

\let\olditemize\itemize
\renewcommand{\itemize}{
  \olditemize
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  (RE)NEW COMMANDS  %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% FOR `NOT SHOUTING' CAPS (e.g. acronyms)
%% ---------------------------------------
\newcommand{\acro}[1]{\textsc{\MakeLowercase{#1}}}    

%% COMMON PHYSICS MACROS
%% ---------------------
\renewcommand{\tilde}{\widetilde}   % tilde over characters
\renewcommand{\vec}[1]{\mathbf{#1}} % vectors are boldface
\newcommand{\dbar}{d\mkern-6mu\mathchar'26}    % for d/2pi
\newcommand{\ket}[1]{\left|#1\right\rangle}    % <#1|
\newcommand{\bra}[1]{\left\langle#1\right|}    % |#1>

%% UNCOMMON PHYSICS MACROS
%% ----------------------
% \newcommand{\CM}[1]{\left(#1\right)_\text{CM}}
% \newcommand{\NS}[1]{#1}
% \newcommand{\DM}[1]{\left(#1\right)_\text{DM}}

%% COMMANDS FOR TEMPORARY COMMENTS
%% -------------------------------
\newcommand{\comment}[2]{\textcolor{red}{[\textbf{#1} #2]}}
\newcommand{\flip}[1]{{
	\color{green!50!black} \footnotesize [\textbf{\textsf{Flip}}: \textsf{#1}]
	}}
	
\definecolor{nirmal}{rgb}{1,0,1}
\definecolor{nirmalcomment}{rgb}{.4,.5,1}

\newcommand{\nirmal}{\textcolor{nirmal}}
\newcommand{\NRcomment}{\textcolor{nirmalcomment}}

\newcommand{\aniket}[1]{{\color{blue} \textnormal{#1}}}
\newcommand{\AJstrike}[1]{{\color{red!90!black} \textnormal{\sout{#1}}}}
\newcommand{\AJcomment}[1]{{\color{orange!90!black} \footnotesize [\textbf{\textsf{Aniket}}: \textsf{#1}]}}
\newcommand{\AJ}[1]{{\color{green!90!black} \textnormal{#1}}}

%% SPECIAL COMMANDS JUST FOR THIS PAPER
%% Macros for CM frame quantities
%% ------------------------------------
\newcommand{\CM}{\text{\rm \tiny{CM}}}
\newcommand{\Mol}{\text{\rm \tiny{M\o l}}}
\newcommand{\esc}{\text{\rm {esc}}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\kcm}{\vec{k}_\CM}



%% COMMANDS FOR TOP-MATTER
%% -----------------------
\newcommand{\email}[1]{\href{mailto:#1}{#1}}
\newenvironment{institutions}[1][2em]{\begin{list}{}{\setlength\leftmargin{#1}\setlength\rightmargin{#1}}\item[]}{\end{list}}


%% COMMANDS FOR LATEXDIFF
%% ----------------------
%% see http://bit.ly/1M74uwc
%\providecommand{\DIFadd}[1]{{\protect\color{blue}#1}} %DIF PREAMBLE
%\providecommand{\DIFdel}[1]{{\protect\color{red}\protect\scriptsize{#1}}}
\providecommand{\DIFadd}[1]{{\protect\color{blue}#1}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{\protect{#1}}}}

%% REMARK: use latexdiff option --allow-spaces
%% for \frac, ref: http://bit.ly/1iFlujR


%%%%%%%%%%%%%%%%%%%
%%%  HYPERREF  %%%%
%%%%%%%%%%%%%%%%%%%

%% This package has to be at the end; can lead to conflicts
\usepackage[
	colorlinks=true,
	citecolor=green!50!black,
	linkcolor=NavyBlue!75!black,
	urlcolor=green!50!black,
	hypertexnames=false]{hyperref}


%%%%%%%%%%%%%%%%%%%%%
%%%  TITLE DATA  %%%%
%%%%%%%%%%%%%%%%%%%%%

%% PREPRINT NUMBER USING fancyhdr
%% Don't forget to set \thispagestyle{firststyle}
%% ----------------------------------------------
\renewcommand{\headrulewidth}{0pt} 	% no separator
\setlength{\headheight}{15pt} 		% min to avoid fancyhdr warning
\fancypagestyle{firststyle}{
	\rhead{\footnotesize%
	\texttt{UCR-TR-2019-FLIP-NCC-1701-C}%
	}}

%% TOC overwrites fancyhdr, here's a fix
%% http://tex.stackexchange.com/questions/167828/
\usepackage{etoc}
\renewcommand{\etocaftertitlehook}{\pagestyle{plain}}
\renewcommand{\etocaftertochook}{\thispagestyle{firststyle}}
